Revisiting Transformer-based Models for Long Document Classification

The recent literature in text classification is biased towards short text sequences (e.g., sentences or paragraphs). In real-world applications, multi-page multi-paragraph documents are common and they cannot be efficiently encoded by vanilla Transformer-based models. We compare different Transformer-based Long Document Classification (TrLDC) approaches that aim to mitigate the computational overhead of vanilla transformers to encode much longer text, namely sparse attention and hierarchical encoding methods. We examine several aspects of sparse attention (e.g., size of local attention window, use of global attention) and hierarchical (e.g., document splitting strategy) transformers on four document classification datasets covering different domains. We observe a clear benefit from being able to process longer text, and, based on our results, we derive practical advice of applying Transformer-based models on long document classification tasks.

==> misc.tex <==
\newpage
\onecolumn
\section{Full results, which will not be included in the paper}

\newpage

\subsection{Table~\ref{table-data-statistics}}

\begin{table}[h!]
    \centering
    %\small
    %\setlength{\tabcolsep}{3pt} % Default value: 6pt
    \begin{tabular}{r rrr}
    \toprule
    & Train & Dev & Test\\
    \midrule
    \bf MIMIC-III (50) \\
\# Documents & 8,066 & 1,573 & 1,729 \\
\# Unique labels & 50 & 50 & 50 \\
\# Avg. words & 1,833 & 2,177 & 2,210 \\
\# Avg. subtokens & 2,260 & 2,693 & 2,737 \\
\# 90th pctl. subtokens & 3,757 & 4,078 & 4,216 \\
    \midrule
    \bf MIMIC-III (Full) \\
\# Documents & 47,719 & 1,631 & 3,372 \\
\# Unique labels & 8,685 & 3,009 & 4,075 \\
\# Avg. words & 1,776 & 2,158 & 2,168 \\
\# Avg. subtokens & 2,186 & 2,668 & 2,682 \\
\# 90th pctl. subtokens & 3,651 & 4,063 & 4,125 \\
    \midrule
    \bf ECtHR \\
\# Documents & 9,000 & 973 & 986 \\
\# Unique labels & 10 & 10 & 10 \\
\# Avg. words & 1,907 & 2,125 & 2,284 \\
\# Avg. subtokens & 2,133 & 2,345 & 2,532 \\
\# 90th pctl. subtokens & 4,750 & 4,930 & 5,576 \\
    \midrule
    \bf 20 Newsgroups \\
\# Documents & 10,183 & 1,131 & 7,532 \\
\# Unique labels & 20 & 20 & 20 \\
\# Avg. words & 484 & 501 & 436 \\
\# Avg. subtokens & 613 & 627 & 551 \\
\# 90th pctl. subtokens & 877 & 895 & 877 \\
    \midrule
    \bf arXiv-11 \\
\# Documents & 23,372 & 5,008 & 5,008 \\
\# Unique labels & 11 & 11 & 11 \\
\# Avg. words & 16,263 & 16,074 & 16,318 \\
\# Avg. subtokens & 18,787 & 18,592 & 18,839 \\
\# 90th pctl. subtokens & 33,772 & 34,466 & 34,445 \\
    \midrule
    \bf Hyperpartisan \\
\# Documents & 516 & 64 & 65 \\
\# Unique labels & 2 & 2 & 2 \\
\# Avg. words & 676 & 648 & 774 \\
\# Avg. subtokens & 741 & 707 & 845 \\
\# 90th pctl. subtokens & 1,530 & 1,566 & 1,833 \\
    \bottomrule
    \end{tabular}
    \caption{Statistics of the datasets. The number of words and subtokens is calculated using RoBERTa tokenizer.}
\end{table}

\newpage

\subsection{Figure~\ref{figure-sequence-length-distribution}}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{images/full_results_sequence_length_distribution_1.pdf}
    \caption{The distribution of document lengths. A log-$10$ scale is used for the X axis.}
\end{figure}

\begin{figure}[h!]
    \centering
    \includegraphics[width=\linewidth]{images/full_results_sequence_length_distribution_2.pdf}
    \caption{The distribution of document lengths.}
\end{figure}


\newpage

\subsection{Hyperpartisan}

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
    \toprule
    \bf Method & \bf F1 \\
    \midrule
    RoBERTa-base (first 512 tokens) & 83.7 \tiny $\pm$ 2.8 \\ % 2022-01-12-A
    RoBERTa-base (Table 7 in beltagy-2020-longformer) & 87.4 \\
    Longformer-base (Table 7 in beltagy-2020-longformer) & 94.8  \\
    \midrule
    \bf Method & \bf Accuracy \\
    \midrule
    RoBERTa-base (first 512 tokens) & 87.2 \tiny $\pm$ 2.1 \\ % 2022-01-12-A
    \bottomrule
    \end{tabular}
    \caption{Dev Results}
\end{table}

\begin{table}[h!]
    \centering
    \begin{tabular}{c|c}
    \toprule
    \bf Method & \bf F1 \\
    \midrule
    RoBERTa-base (first 512 tokens) & 95.5 \tiny $\pm$ 1.6 \\ % 2022-01-12-A
    \midrule
    \bf Method & \bf Accuracy \\
    \midrule
    RoBERTa-base (first 512 tokens) & 96.3 \tiny $\pm$ 1.2 \\ % 2022-01-12-A
    \bottomrule
    \end{tabular}
    \caption{Test Results}
\end{table}

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{images/20210907A.pdf}
    \caption{Concatenating the hidden states of [CLS] token and the most five informative wordpieces, identified using TF-IDF.}
\end{figure}

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{images/20210914A.pdf}
    \caption{Randomly choose in-vocabulary words (not stop-words) and forcefully segment them into multiple wordpieces.}
\end{figure}

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{images/20210821.pdf}
    \caption{Keep only the first 3 wordpieces of these over-segmented words.}
\end{figure}

\begin{figure}[b]
    \centering
    \includegraphics[width=\linewidth]{images/20210930C-1.png}
    \caption{Using the first 1024 wordpieces seems to be good enough in EURLEX57K.}
\end{figure}

\subsection{Recurrent Transformers}

In another direction, recurrent transformers have been introduced as an alternative to process longer documents and improve contextualization.

\textbf{Transformer-XL} of \citet{dai-2019-acl-transformer-xl}  extends Transformer-based models to support longer sequences by using a recurrent memory. The model encodes tokens in segments, where tokens co-attend each other. In addition, each segment re-uses hidden states from the previous segment as memory for the current segment, which builds up a recurrent connection along the segments. In this fashion, the model can capture very long-term dependencies because information can be propagated through the recurrent connections. Furthermore, in order to apply Transformer-XL to longer sequences, \citeauthor{dai-2019-acl-transformer-xl} introduce relative positional encodings used to describe the relative position of one token to another in the attention.

\cite{ding-2021-acl-ernie-document} X \\ X \\ X \\ X \\ X \\ X \\ X \\ X \\ X \\ X \\ X \\ X \\ X \\

==> response.tex <==
\section{Author Response}

\paragraph{Meta Reviewer DQzP.}\hspace{-1em} We are surprised by the Suggested Revisions from Area Chair \texttt{DQzP}. In our June 2022 submission, we believe that we addressed the major concerns raised by Area Chair \texttt{ifLw} w.r.t.\ our November 2021 submission. The new Meta Review from \texttt{DQzP} says the paper could be improved by ``figuring out more consistent results and which practical strategy (or combination of strategies) is most beneficial on the long document classification task''. At a conceptual level, we respectfully disagree that researchers should expect to always figure out consistent results from purely empirical studies. It may be that there is no ``consistent result'' that can be found from four such different datasets, as highlighted in Q1 (L450--456). Furthermore, we have already added a new section of Practical Advice (L446--476).

We discuss these concerns in more detail:

\begin{quote}
    Comment: “difficult to figure out the consistent results and the practical strategy”
\end{quote}

We conduct a series of controlled experiments on four datasets covering three different domains (clinical notes, legal cases, news articles) to understand the impact of design choices in different long document classification models. 
Our results suggest that, on one hand, some design choices are robust and same patterns are observed across different datasets (e.g., size of local attention window; chosen tokens with global attention); on the other hand, some choices (e.g., document splitting strategy in hierarchical method) are dataset dependent.

We cannot suggest a one-fit-all solution for all datasets, especially when these datasets vary in terms of domain, style, and document length. Instead, we suggest starting points for practitioners who do not plan on extensively tuning hyperparameters and identify design choices that may benefit from careful hyperparameter tuning.

\begin{quote}
    Comment: “suggested advice should take into account the resources constraints”
\end{quote}

We show a comparison between Longformer and Hierarchical models regarding the number of parameters and their GPU consumption in Appendix 9.9 and Table 8.
We will move these contents to the main text and update our practical advice under different resource constraints.

\paragraph{Reviewer E5G1} \hspace{-1em} asks for additional details on the computation complexity of using Transformer-based models for long-document classification. We already report some information in Table 1 (speed efficiency) and in Table 8 (GPU memory usage) of our models. We can add similar analyses of RNN-based models when we revise the paper.

\paragraph{Reviewer 2vkB} \hspace{-1em} notes, as a weakness, that we did not report or discuss the results on the Hyperpartisan or 20 News datasets, as promised in the author response. This is not accurate. The results can be found in Table 3 and the discussion on L422--433.

\paragraph{Reviewer VPyY} \hspace{-1em} is concerned that the considered models do not improve on the Hyperpartisan or 20 News datasets. We included these experiments to address a ``generalization concern'' of Area Chair \texttt{ifLw}. The models in our experiments were specifically designed to deal with long documents, but neither of those datasets actually contain long documents compared to MIMIC-III or ECtHR (see Table 4). The empirical results in Table 3 support this claim: there is little difference between processing the whole document or the fist 512 tokens for the 20 News dataset.

\clearpage

\section{Limitations}
Long document classification datasets are usually annotated using a large number of labels. 
For example, the complete MIMIC-III dataset contains nearly 9,000 unique labels, and the ECtHR dataset contains 40 unique labels. 
As we mentioned in Section 2, we focus on building document representation using Transformer-based models and leave the challenge of learning with a large target label set for future work.
Therefore, in this paper, we follow previous work~\citep{mullenbach-gatech-2018-naacl-caml,chalkidis-jana-2022-acl-lexglue} and consider a subset of frequent labels only. That is, we use the top 50 frequent labels in MIMIC-III and 10 labels in ECtHR.



